Nonlinear Invariant Risk Minimization: A Causal Approach

Due to spurious correlations, machine learning systems often fail to generalize to environments whose distributions differ from the ones used at training time. Prior work addressing this, either explicitly or implicitly, attempted to find a data representation that has an invariant relationship with the target. This is done by leveraging a diverse set of training environments to reduce the effect of spurious features and build an invariant predictor. However, these methods have generalization guarantees only when both data representation and classifiers come from a linear model class. We propose invariant Causal Representation Learning (iCaRL), an approach that enables out-of-distribution (OOD) generalization in the nonlinear setting (i.e., nonlinear representations and nonlinear classifiers). It builds upon a practical and general assumption: the prior over the data representation (i.e., a set of latent variables encoding the data) given the target and the environment belongs to general exponential family distributions. Based on this, we show that it is possible to identify the data representation up to simple transformations. We also prove that all direct causes of the target can be fully discovered, which further enables us to obtain generalization guarantees in the nonlinear setting. Extensive experiments on both synthetic and real-world datasets show that our approach outperforms a variety of baseline methods. Finally, in the discussion, we further explore the aforementioned assumption and propose a more general hypothesis, called the Agnostic Hypothesis: there exist a set of hidden causal factors affecting both inputs and outcomes. The Agnostic Hypothesis can provide a unifying view of machine learning. More importantly, it can inspire a new direction to explore a general theory for identifying hidden causal factors, which is key to enabling the OOD generalization guarantees.

==> fig4.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.4\textwidth}
\centering
\begin{tikzpicture}[
	> = latex, % arrow head style: triangle 45, latex, stealth
    auto,
    observed/.style={circle, draw=black, fill=black!15, thick, inner sep=0pt, minimum size=6mm},
    unobserved/.style={circle, draw=black, thick, inner sep=0pt, minimum size=6mm},
    surrogate/.style={rectangle, draw=black, fill=black!15, thick, minimum size=5mm},
]        
		
		\node[unobserved] (X1) {\tiny $X_1$};
		\node[unobserved] (X2) [right=0.6cm of X1] {\tiny $X_2$};
        \node[observed] (Y) [right=0.6cm of X2] {\tiny $Y$};
        \node[surrogate] (E) [above=0.6cm of Y] {\tiny $E$};
        \node[observed] (X) [below=0.6cm of Y] {\tiny $\boldsymbol{O}$};
       
        \path[->, very thick] (X1) edge [bend right=45] (Y);
        \path[->, very thick] (X2) edge (Y);
        \path[->, very thick] (E) edge (X1);
        \path[->, very thick] (E) edge (X2);
		\path[->, very thick] (X1) edge (X);
		\path[->, very thick] (X2) edge (X);
        
\end{tikzpicture}
\caption{} 
\label{fig:main_two_causes_g}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
\centering
\begin{align}
    E &\sim \mathcal{U}\left\{0.2, 2, 3, 5\right\} \\
    X_1 &\sim \mathcal{N}(X_1 | E, 1) \\
    X_2 &\sim \mathcal{N}(X_2 | 2E, 2) \\
    Y &\sim \mathcal{N}(Y | X_1 + X_2, 1) \\
    \boldsymbol{O} &= g(X_1, X_2)
\end{align}
\caption{} 
\label{fig:main_two_causes_dg}
\end{subfigure}
\caption{(a) Causal structure with $Y$ having two causes. (b) Data generating process corresponding to (a), where $\mathcal{U}\{\cdot\}$ denotes the discrete uniform distribution, $\mathcal{N}(\cdot)$ the Gaussian distribution, and $g(\cdot)$ is given by a neural network with 2-dimensional input and 10-dimensional output, whose parameters are randomly set in advance.} \label{fig:main_two_causes}
\end{figure}


==> fig5.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/scatter_gt.pdf}
\caption{Data generating model}
\label{fig:main_2a}
\end{subfigure}%
\begin{subfigure}{.7\textwidth}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Row %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/scatter_vae.pdf}
\caption{VAE}
\end{subfigure}%
\hspace{2mm}
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/scatter_ivae.pdf}
\caption{iVAE}
\end{subfigure} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Row %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/scatter_icebeem.pdf}
\caption{ICE-BeeM}
\end{subfigure}%
\hspace{2mm}
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/scatter_icarl.pdf}
\caption{iCaRL-iVAE}
\end{subfigure}

\end{subfigure}
\caption{Visualization of the samples (i.e., $\hat{\boldsymbol{X}}=(\hat{X}_1, \hat{X}_2)$) in latent space generated through different algorithms. (a) Samples from the true distribution. (b-e) Samples from the posterior of different algorithms. Apparently, our method (e) can recover the original data up to a permutation and a simple componentwise transformation.} 
\label{fig:main_idf_visualization}
\end{figure}


==> tab_fashion_vlcs.tex <==
\begin{table}[t] \vspace{-4mm}
\centering
\begin{minipage}{.48\textwidth} 
\centering
\caption{\footnotesize Colored Fashion MNIST. Comparisons in terms of accuracy (\%) (mean $\pm$ std deviation).} \vspace{-2mm}
\label{tab:fashion} 
\LARGE
\begin{adjustbox}{width=0.95\columnwidth,center}
\begin{tabular}{@{\hspace{0.01cm}}lcc@{\hspace{0.01cm}}}
\multicolumn{1}{c}{\bf METHOD}  &\multicolumn{1}{c}{\bf TRAIN } &\multicolumn{1}{c}{\bf TEST }
\\ \hline \vspace{-6mm}\\
ERM                 & $83.17 \pm 1.01$ & $22.46 \pm 0.68$ \\
ERM 1               & $81.33 \pm 1.35$ & $33.34 \pm 8.85$\\
ERM 2               & $84.39 \pm 1.89$ & $13.16 \pm 0.82$ \\
ROBUST MIN MAX      & $82.81 \pm 0.11$ & $29.22 \pm 8.56$ \\
F-IRM GAME          & $62.31 \pm 2.35$ & $69.25 \pm 5.82$ \\
V-IRM GAME          & $68.96 \pm 0.95$ & $70.19 \pm 1.47$ \\
IRM                 & $75.01 \pm 0.25$ & $55.25 \pm 12.42$ \\
{\bf iCaRL (ours)}          & $\boldsymbol{74.96 \pm 0.37}$ & $\boldsymbol{73.61 \pm 0.63}$ \\
ERM GRAYSCALE       & $74.79 \pm 0.37$ & $74.67 \pm 0.48$ \\
OPTIMAL             & $75$ & $75$ \\ \hline \vspace{-6mm}
\end{tabular}
\end{adjustbox}
\end{minipage}\hspace{4mm}%
\begin{minipage}{.48\textwidth} 
\centering 
\caption{\footnotesize VLCS. Comparisons in terms of accuracy (\%) (mean $\pm$ std deviation).} \vspace{-2mm}
\label{tab:vlcs}
\LARGE
\begin{adjustbox}{width=0.80\columnwidth,center}
\begin{tabular}{@{\hspace{0.01cm}}lcc@{\hspace{0.01cm}}}
\multicolumn{1}{c}{\bf METHOD}   &\multicolumn{1}{c}{\bf TEST }
\\ \hline \vspace{-6mm}\\
ERM               & $77.4 \pm 0.3$ \\
IRM               & $78.1 \pm 0.0$ \\
DRO \citep{sagawa2019distributionally}& $77.2 \pm 0.6$ \\
Mixup \citep{yan2020improve} & $77.7 \pm 0.4$ \\
CORAL \citep{sun2016deep}   & $77.7 \pm 0.5$ \\
MMD \citep{li2018domain}    & $76.7 \pm 0.9$ \\
DANN \citep{ganin2016domain} & $78.7 \pm 0.3$ \\
C-DANN \citep{li2018deep}   & $78.2 \pm 0.4$ \\
LaCIM \citep{sun2020latent} & $78.4 \pm 0.5$ \\
{\bf iCaRL (ours)}& $\boldsymbol{81.8 \pm 0.6}$ \\ \hline \vspace{-7mm}
\end{tabular}
\end{adjustbox}
\end{minipage} 
\end{table}



